Scale Can't Overcome Pragmatics: The Impact of Reporting Bias on Vision-Language Reasoning

The lack of reasoning capabilities in Vision-Language Models (VLMs) has remained at the forefront of research discourse. We posit that this behavior stems from a reporting bias in their training data. That is, how people communicate about visual content by default omits tacit information needed to supervise some types of reasoning; e.g., "at the game today!" is a more likely caption than "a photo of 37 people standing behind a field". We investigate the data underlying the popular VLMs OpenCLIP, LLaVA-1.5 and Molmo through the lens of theories from pragmatics, and find that reporting bias results in insufficient representation of four reasoning skills (spatial, temporal, negation, and counting), despite the corpora being of web-scale, and/or synthetically generated. With a set of curated benchmarks, we demonstrate that: (i) VLMs perform poorly on the aforementioned types of reasoning suppressed in the training data by reporting bias; (ii) contrary to popular belief, scaling data size, model size, and to multiple languages does not result in emergence of these skills by default; but, promisingly, (iii) incorporating annotations specifically collected to obtain tacit information is effective. Our findings highlight the need for more intentional training data curation methods, rather than counting on scale for emergence of reasoning capabilities.

==> 7_discussion.tex <==


% \section{\new{\textit{Can} models reason, if reporting bias was mitigated?}}
% \label{sec:finetuning}
% Our experiments show strong evidence that reporting bias causes low occurrence of reasoning-related concepts in training data, which in turn correlates with poor model performance on corresponding types of reasoning. To cement reporting bias as a cause of poor VLM reasoning, we ask the question: if given data in which this reporting bias were mitigated, i.e., data with higher representation of reasoning-related concepts, does VLM reasoning performance improve?

% Answering this question would require the creation of
% % The true control for this experiment would be to create 
% a large-scale vision-language pretraining dataset collected with our recommended annotator instructions, or via other methods that mitigate reporting bias. Unfortunately, this is beyond our resources. 
% Instead, we run small-scale finetuning experiments, to determine whether VLMs are capable of the tasks we evaluate them on.

% We first curate a dataset with counting data equivalent to the percentage occurrence of counting data we surface with ``our'' annotation instructions in Section \ref{sec:controlled_study}, i.e., 39\%.
% To achieve this, we sample a balanced subset of counting data from TallyQA (1000 examples per count between 2--10) and combine it with the corresponding proportion of LLaVA-1.5 instruction tuning data (which we estimate to have 6.9\% counting data\footnote{This is a subset of the LLaVA-1.5 training data studied in Section \ref{sec:counts}, and thus has a slightly different occurrence rate for counting than is reported in Table \ref{tab:occurrence}.}).
% % To achieve this, we calculate the amount of counting data in LLaVA-1.5 instruction tuning data (estimated at 6.9\%\footnote{This is a subset of the LLaVA-1.5 training data studied in Section \ref{sec:counts}, and thus has a slightly different occurrence rate for counting than is reported in Table \ref{tab:occurrence}.}) and combine it with a balanced subset of counting data from TallyQA (1000 examples per count between 2 and 10). 
% In total, we combine 9,000 data points from TallyQA with 17,138 data points from LLaVA-1.5 instruction tuning data, to obtain a corpus of about 26K examples with 39\% occurrence of counting data. 

% We finetune LLaVA-1.5-13b on this data for 1 epoch on 2 L40S GPUs at a batch size of 4 and learning rate of 1e-6, then evaluate the finetuned model on our counting benchmark from Section \ref{sec:benchmarks}. 
% % The finetuned model's performance on our counting benchmark is 54.4\%, which is 5.5 points higher than the base model performance at 48.9\%. 
% To ensure the proportion of counting concepts in the finetuning data was indeed the cause of this gain, we compare to finetuning LLaVA-1.5-13b on a corpus of the same size with less occurrence of counting data, i.e., only LLaVA instruction tuning data.
% Our results are shown in Table \ref{tab:finetuning}: finetuning on data without reporting bias outperforms both the base model, and finetuning on data with reporting bias.

% While
% % While this is not as tight of a control (
% finetuning on a distribution of data without reporting bias, i.e., with high representation of reasoning-related concepts, unsurprisingly increases model performance on those types of reasoning, 
% this experiment does show that: 
% (1) these types of reasoning are not precluded by the architecture of these models, which agrees with our results from Table 2 and findings from \citet{paiss2023teaching};
% and (2) our annotator instructions surface sufficient representation of reasoning-heavy concepts (here, counting) for the model to learn the task, i.e., they successfully mitigate reporting bias.

% While the latter finding has promising implications for data collection methods, the significant gap between the finetuned model and human performance reported in Table \ref{tab:main_results} highlights room for improvement---underscoring the importance of mitigating reporting bias while collecting pretraining corpora for VLMs. 

% \input{tables/finetuning}

==> old/abstract_v1.tex <==
\begin{abstract}
% Despite surpassing human performance on many standard benchmarks,
Vision-language models (VLMs) consistently exhibit
poor performance on simple tasks
%basic for humans
like spatial reasoning and counting. % \jack{can we be more direct here with an example?}
% Language: correlates instead of "stems from"/"is caused by"?
We posit that this behavior stems from a \emph{reporting bias} in vision-language pretraining data. That is, % that the human behaviors contributing to 
how people communicate using images by default omits %results in the systematic omission of certain types of
information needed to supervise some types of reasoning, e.g., ``at the game today!'' is a more likely caption than ``A photo of 37 people standing behind the field.'' % \jack{this aside might be doing too much, but I wanted to give a specific vibe early on. :P }
% Repeated
% --- regardless of the scale of the model or training data. 
In this work,
we investigate the pragmatics of the data % four such types of omitted information in
underlying popular image-text models like OpenCLIP, LLAVA-1.5 and Molmo, and find that four reasoning skills (spatial, temporal, negation, and counting) are not well represented. % required for image-text learning. 
% We find four alongside explanations thereof rooted in pragmatics and cognitive science.
A set of reframed benchmarks demonstrates that: i) frequency of skill-requiring instances predicts model performance; ii) scaling data size, model size, and to multiple languages does \emph{not} result in emergence of these skills; but, promisingly, iii) incorporating annotations specifically collected to operationalize the naturally omitted information is effective. %improve model performance. \jack{A takeaway: supervision specifically targeted towards ``patching"} % We release code+data. %\jack{} help future supervised data collection efforts
We release code+data, along with experiments on eliciting reasoning-related information from annotators.

% We curate benchmarks evaluating each of these four types of reasoning, and show that top-performing contrastive and generative VLMs all perform poorly.
% This sentence feels out of place:
% We show that reporting bias occurs unless training data annotators are specifically prompted to discuss the omitted information, and predicts corresponding model performance. 
% Further, we show that neither scaling up the model size, training data size, nor multilingual diversity in the training data significantly improves model performance, which highlights the need for reasoning-aware data collection.
% We close with a discussion on closed-source VLMs, which also leave room for improvement.
% We release the evaluation data and code to encourage the research community to focus on data quality in addition to scale. 
\end{abstract}
